Refine-Net: Normal Refinement Neural Network for Noisy Point Clouds

Point normal, as an intrinsic geometric property of 3D objects, not only serves conventional geometric tasks such as surface consolidation and reconstruction, but also facilitates cutting-edge learning-based techniques for shape analysis and generation. In this paper, we propose a normal refinement network, called Refine-Net, to predict accurate normals for noisy point clouds. Traditional normal estimation wisdom heavily depends on priors such as surface shapes or noise distributions, while learning-based solutions settle for single types of hand-crafted features. Differently, our network is designed to refine the initial normal of each point by extracting additional information from multiple feature representations. To this end, several feature modules are developed and incorporated into Refine-Net by a novel connection module. Besides the overall network architecture of Refine-Net, we propose a new multi-scale fitting patch selection scheme for the initial normal estimation, by absorbing geometry domain knowledge. Also, Refine-Net is a generic normal estimation framework: 1) point normals obtained from other methods can be further refined, and 2) any feature module related to the surface geometric structures can be potentially integrated into the framework. Qualitative and quantitative evaluations demonstrate the clear superiority of Refine-Net over the state-of-the-arts on both synthetic and real-scanned datasets. Our code is available at https://github.com/hrzhou2/refinenet.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> approach.tex <==
%\section{Overview}
%We propose a two-step normal estimation method via the collaboration of a geometric estimator and a deep network called NH-Net. Fig. \ref{fig:pipeline} shows an overview of the proposed approach. It consists of the following two main steps: multi-scale suboptimal normal estimation (MSNE) and NH-Net. First, we propose a multi-scale fitting patch selection (MFPS) for each candidate point (near sharp feature) to compute its suboptimal normal, while obtaining the suboptimal normals for smooth points (far from sharp features) via PCA (Sec. 4). Then, based on these computed normals, we define a multi-scale point descriptor (MPD) via bilateral normal filter (BNF) for each point as the input of the following network (Sec. 5.1).  Ultimately, we recover the final optimal normals by our NH-Net, containing two sub-modules, namely a height-map patch (HMP) based improving module and a gathering module (Sec. 5.2).


\begin{figure}
	\begin{center}
		\includegraphics[width=0.24\linewidth]{fig/plane_cmp/input1.pdf}
		\includegraphics[width=0.24\linewidth]{fig/plane_cmp/RNE1.pdf}
		\includegraphics[width=0.24\linewidth]{fig/plane_cmp/PCV1.pdf}
		\includegraphics[width=0.24\linewidth]{fig/plane_cmp/ours1.pdf}
		\vspace{-2pt}
		\subfigure[Noisy input]{
			\label{fig:plane_cmp:input} %% label for first subfigure
			\includegraphics[width=0.23\linewidth]{fig/plane_cmp/input3.pdf}}
		\subfigure[RNE \cite{li2010robust}]{
			\label{fig:plane_cmp:RNE} %% label for first subfigure
			\includegraphics[width=0.23\linewidth]{fig/plane_cmp/RNE3.pdf}}
		\subfigure[PCV \cite{zhang2018multi}]{
			\label{fig:plane_cmp:PCV} %% label for first subfigure
			\includegraphics[width=0.23\linewidth]{fig/plane_cmp/PCV3.pdf}}
		\subfigure[Ours]{
			\label{fig:plane_cmp:ours} %% label for first subfigure
			\includegraphics[width=0.23\linewidth]{fig/plane_cmp/ours3.pdf}}
		
	\end{center}
	\caption{Comparison of the selected planes by different methods. From the left column to the rightmost: Noisy input, and the plane fitting results of RNE, PCV and our method. Red points represent the noisy input and blue star in the first column is the target point. The green line means the selected plane and the blue points are neighbors considered to fit this plane in the corresponding method. We can easily observe that our method can select the most suitable plane, with the help of better neighboring information.}
	\label{fig:plane_cmp}
\end{figure}


%-------------------------------------------------
\section{Multi-scale suboptimal normal estimation}
\label{sec:geometric}
Before computing the initial normal for each point, we first apply the local covariance analysis (Sec. 4.2 in \cite{zhang2013point}), to classify all points into candidate points (near sharp features) and smooth points (far from sharp features). The normals of smooth points can be simply computed by PCA.

To estimate the normals for candidate points, one common strategy is to randomly select three non-collinear points to construct a set of candidate planes and pick up one that best describes the underlying surface patch. Typical methods are RNE \cite{li2010robust} and PCV \cite{zhang2018multi}, in which they introduce a residual bandwidth to evaluate proximity of the candidate planes to the underlying surface. However, when they come to noisy inputs, the neighborhood of the target point for detecting candidate plane is often corrupted by points from another side of the intersection. This causes the selected plane deviating from the true surface (Fig.~\ref{fig:plane_cmp:RNE}). PCV is better but still imperfect (Fig.~\ref{fig:plane_cmp:PCV}).


\iffalse
To better evaluate proximity of the selected plane to surrounding neighbors, \cite{li2010robust}(RNE) suggests to use the a residual bandwidth to detect points from the same facet. Their objective function is defined as:
\begin{equation}
\theta_{i}^{*} = \mathop{\arg\max}_{\theta} \frac{1}{\Omega} \sum_{{p}_{i}^{j} \in \mathcal N_{r}(i)} W_{1}(\frac{r_{j,\theta}^{2}}{\sigma_{i}^{2}}),
\end{equation}

where $\theta$ represents a candidate plane randomly selected above, $\mathcal N_{r}(i)$ is the neighborhood of $p_i$, $\Omega$ is a normalization factor, $W_{1}$ is a decreasing weight function, $r_{j,\theta}$ is the distance from point $p_i^j$ to plane $\theta$, $\sigma_{i}$ is the residual bandwidth for $p_i$.
RNE tends to select a plane matching as many points as possible with the constraint of bandwidth $\sigma_{i}$. However, it may fail in the presence of noise and sharp feature since points from different facets contribute equally, see Figure~\ref{fig:plane_cmp:RNE}.
%One reason is that points in different facets contribute equally without any constraint, and consequentially the objective function will perfer planes with slight tendency towards adjacent facets.

In order to reduce the influence of neighbors across edges, \cite{zhang2018multi} (PCV) suggests that the point pairs with similar normals should contribute more, and they propose the following objective function:
\begin{equation}
\theta_{i}^{*} = \mathop{\arg\max}_{\theta} \sum_{{{p}_{i}^{j},{p}_{i}^{j}} \in \mathcal N_{r}(i)} W_2(\frac{r_{j,\theta}^{2}}{\sigma_{i}^{2}}) W_2(\frac{r_{k,\theta}^{2}}{\sigma_{i}^{2}}) \rho({n}_{i}^{j}, {n}_{i}^{k}),
\end{equation}

where $W_2$ is a decreasing gaussian function, $n_i^j, n_i^k$ are the initial normals of $p_i^j, p_i^k$, respectively, computed by PCA, and $\rho$ is a weight function rewarding similar normals.

PCV performs better on points near sharp features due to the underlying facet information implied by normal pairs. However, when it comes to large noise regions, the candidate plane selected by PCV can not accurately describe the true surface, see Fig \ref{fig:plane_cmp:PCV}. If the considered neighborhood is corrupted by points from other sides of the intersection, the estimator has to balance these undesired points. This cause the deviation of estimated normals. On the other hand, preliminary normals $n_i^j, n_i^k$ computed by PCA are unreliable near sharp features.
%The selected plane with highest score (denoted as green line) still has a good performance on the same facet as $p_i$, and simultaneously it tends to balance points on the other side of edge which can get a higher score. On the other hand, preliminary normals $n_i^j, n_i^k$ computed by PCA  are not reliable near sharp features.

%To sum up, these methods are capable of reducing the influence across edges, but can not obtain accurate normals in the presence of large noise. If the estimated points $p_i$ is near sharp features, the commonly chosen neighborhood $\mathcal N_{r}(i)$ might be corrupted by points coming from the wrong side of the edge, resulting in the deviation of estimated normals.
%In the following sections, we will introduce a normal estimation method that is insensitive to sharp features and noise provide suitable and flexible neighbors in both sharp features and smaller features, even with high level noise.
\fi

\subsection{Multi-scale patch detection}
Considering the problems stated above, we propose to select a more consistent and flexible neighborhood which provides better local structure information for robust normal estimation. For each candidate point $p_i$, our method tries to find the best fitting patch that contains $p_i$.
%We first present a simple version followed by the
Please note normals of smooth points are already computed by PCA.

First, for each point $p_j$ in a point cloud, we find several local patches, each defined as $Q_j^t$ (the $K_t$-nearest neighboring points of $p_j$). The patch size $K_t$ is from the scale parameter set $K = \{K_1, K_2, ..., K_a\}$. Rather than detecting patches using a fixed neighborhood size which is commonly used in \cite{li2010robust} and \cite{zhang2018multi}, this multi-scale scheme ensures a robust estimation especially for point clouds with high density variation. Then,  the fitting plane $\theta_{Q_j^t}^{*}$ of each patch $Q_j^t$ is determined by the following objective function:
\begin{equation}
E_{Q_j^t}(\theta) =  \frac{1}{|Q_j^t|} \sum_{{p}_{j}^{k} \in Q_j^t} W_{\sigma_{j}}(p_j^k, \theta),
\end{equation}
\begin{equation}
\theta_{Q_j^t}^{*} = \mathop{\arg\max}_{\theta} E_{Q_j^t}(\theta), \label{equ:patch_plane}
\end{equation}
where $W_{\sigma_{j}}(p_j^k, \theta) = exp(- r_{k,\theta}^2 / \sigma_{j}^2)$ is the Gaussian function in which $r_{k,\theta}$ denotes the distance from point $p_j^k$ to the plane $\theta$, and $\sigma_{j}$ is the residual bandwidth of $p_j$.

Denote $S_{i} = \{Q_j^t | p_i \in Q_j^t \} $ as all patches containing candidate point $p_i$. We aim to search for, among all patches in $S_i$, the most isotropic one and to use the normal of the fitting plane of this patch as the suboptimal normal of $p_i$. As shown in Fig.~\ref{fig:pipeline} (the MSNE part), the multi-scale approach makes more candidate patches available in $S_i$ in order to promote the robustness to strong noise and details (see from Fig.~\ref{fig:plane_cmp:ours}), in which the scale parameter is set as $K = 50, 100, 150$ by default in our experiments. 

Thus, the fitting patch selection process for $p_i$ is performed completely within $S_{i}$ by measuring the consistency of these patches:
\begin{equation}
\mathcal D(Q_j^t) = E_{Q_j^t}(\theta_{Q_j^t}^{*}) \eta(K_t). \label{equ:point_plane}
\end{equation}
where
\[ \eta(K_t) = \alpha + (1-\alpha) \frac{K_t-K_{min}}{K_{max}-K_{min}}\]
Here, $\theta_{Q_j}^{*}$ is the fitting plane of $Q_j$ determined by Eq.~\ref{equ:patch_plane}. The larger $ E_{Q_j}(\theta_{Q_j}^{*})$ is, the smaller the plane fitting error is, and $\eta(K_t)$ is a tradeoff parameter used to punish relately small patches because larger ones are preferred in noisy areas. We set $\alpha=0.9$ empirically. 
%$\mathcal D_i$, therefore, represents the most precise patch within $S_{p_i}$ for $p_i$, and we use the normal of the fitting plane of this patch as the suboptimal normal of candidate point $p_i$.




\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.99\linewidth]{fandisk.pdf}
	\end{center}
	\caption{Visual comparison of estimated normals on noisy fandisk model (without point update). From left to right: noisy input, our NH-Net trained on PCA normals, suboptimal normals without the network, and our NH-Net trained on suboptimal normals.}
	\label{fig:pca_cmp}
\end{figure}



\subsection{Best-fitting patch selection}
Given all the optional patches (along with their normals) in $S_i$, commonly we select the one with maximum evaluation value $\mathcal D(Q_j^t)$ as the best-fitting patch to determine the suboptimal normal for candidate point $p_i$. However, if $p_i$ lies closely in the neighborhoods of sharp features, the resulting normal might be in an undesired direction where the underlying surface is more consistent with a higher point density level. This may cause a large angular error on sharp edges (see Fig.~\ref{fig:fps:gt}), which can not be modified in the following refine network. Inspired by \cite{sanchez2020robust}, we sort the candidate patches in $S_i$ by their consistency measurement $\mathcal D(Q_j^t)$ and select several anisotropic patches starting with the largest $\mathcal D(Q_j^t)$. 
%First, for each patch $Q_j \in S$, we find a reference point $p^{\textbf{ref}}_j$ by projecting $p_i$ onto its fitting plane $\theta_{Q_j}^*$ determined by Eq.~\ref{equ:patch_plane}. Then, the normal $n(\theta_{Q_j}^*)$ is reoriented to the exterior of the surface, which means it must satisfy the following condition:
%\begin{equation}
%\sum_{p_k \in N_i} n(\theta_{Q_j}^*) \cdot (p_i - p_k) < 0,
%\end{equation}
%Here, $N_i$ is the neighborhood of $p_i$. 
Specifically, our method adds a new patch $Q \in S_i$ and its corresponding normal to the anisotropic patch set $A_i = \{(Q_1^{\textbf{ani}}, n_1^{\textbf{ani}}), (Q_2^{\textbf{ani}}, n_2^{\textbf{ani}}), ...\}$, if $D(n_Q, n_j^{\textbf{ani}}) > w_t, \forall j$, where $n_Q$ is the normal of fitting plane of $Q$, metric $D$ is calculated as the angular error of two normals and $w_t$ is an angular threshold. In our experiments, we set $w_t$ to $60^{\circ}$.

The final step is to choose one patch from $A_i$, which can best describe the underlying surface of $p_i$. First, for each patch $Q_j^{\textbf{ani}} \in A_i$, we find a reference point $p^{\textbf{ref}}_j$ by projecting $p_i$ onto its fitting plane $\theta_{Q_j^{\textbf{ani}}}^*$ determined by Eq.~\ref{equ:patch_plane}:
\begin{equation}
p^{\textbf{ref}}_j = p_i + r_{i,\theta} \cdot n_j^{\textbf{ani}},
\end{equation}
where $r_{i,\theta}$ is the signed distance from target point $p_i$ to $\theta_{Q_j^{\textbf{ani}}}^*$.
Secondly, normal $n_j^{\textbf{ani}}$ is reoriented to the exterior of the surface, which means it must satisfy the following condition:
\begin{equation}
\sum_{p_k \in N_i} n_j^{\textbf{ani}} \cdot (p^{\textbf{ref}}_j - p_k) < 0. 
\end{equation}
Here, $N_i$ is the neighborhood of $p_i$. 
%Secondly, the reference point $p^{\textbf{ref}}_j$ is computed according to the corresponding patch $Q_j^{\textbf{ani}}$:
%\begin{equation}
%p^{\textbf{ref}}_j = p_i + \frac{1}{|Q_j|} \sum_{p_k \in Q_j^{\textbf{ani}}}  (p_i - p_k) {n_j^{\textbf{ani}}}^T n_j^{\textbf{ani}},
%\end{equation}
%where $Q_j^{\textbf{ani}}$ denotes the points within this patch. 
Similar to \cite{sanchez2020robust}, values $\{n_j^{\textbf{ani}} \cdot (p^{\textbf{ref}}_j - p_i)\}(j=1,2,...)$ are computed, and the minimum value corresponds to the suboptimal normal of $p_i$. A detailed explanation is given in Fig.~\ref{fig:fps}. Note that, $p^{\textbf{ref}}_j$ is only used for patch selection, which is not a new point in the point cloud.

The output suboptimal normals will be used in the following NH-Net which can preserve geometric features as shown in the third sub-figure of Fig.~\ref{fig:pca_cmp}. These initial normals enhance the performance of the network compared with directly using raw normals (PCA) as input, see Fig.~\ref{fig:pca_cmp}.


\begin{figure}
	\begin{center}
		\hspace{-8pt}
		\subfigure[Ground truth]{
			\label{fig:fps:gt} %% label for first subfigure
			\includegraphics[width=0.33\linewidth]{fig/fps/fps1.pdf}}
		\hspace{-8pt}
		\subfigure[Anisotropic patch 1]{
			\label{fig:fps:ani1} %% label for first subfigure
			\includegraphics[width=0.33\linewidth]{fig/fps/fps2.pdf}}
		\hspace{-8pt}
		\subfigure[Anisotropic patch 2]{
			\label{fig:fps:ani2} %% label for first subfigure
			\includegraphics[width=0.33\linewidth]{fig/fps/fps3.pdf}}
		
	\end{center}
	\caption{Patch selection for the best-fitting normal of $p_i$ (the green point). (a) represents the input points on a sharp edge and the ground truth normal $N_{GT}$. (b)(c) describe two selected aniostropic normals and their patch points. The black arrow denotes the signed distance from $p_i$ to $p^{\textbf{ref}}_j$, which determines the selected patch (patch 2).}
	\label{fig:fps}
\end{figure}



\section{NH-Net}
In this section, we introduce the learning part in our algorithm pipeline. The network architecture is outlined in Fig. \ref{fig:pipeline} (the purple and green parts). First, we introduce a multi-scale descriptor, called MPD, and then explain how to feed it into the next two-stage learning module which spits out the final normal. The details are followed.

\subsection{MPD: multi-scale point descriptor}
As known, the input data of a neural network should be in a structural format. Inspired by the work in Wang et al. \cite{wang2016mesh}, for each point, we define its MPD by $X$ pairs of filtered normal plus local HMP to collaboratively enhance the learning effect. Filtered normals at each point are computed by bilateral filtering based on the normals estimated in Sec. 4, and the HMPs are constructed according to the corresponding filtered normals.


\subsubsection{Multi-scale bilateral filters:}
We give a brief introduction to the commonly-used bilateral filters \cite{jones2004normal}. Denote the neighborhood of $p_i$ as $N_i$, and the normal at each point as $n_i^{sub}$. The filtered normal can be defined as:
\begin{equation}
n_i = \Lambda(\sum_{{p}_{j}\in N_i} W_s(||p_i-p_j||) W_r(||n_i^{sub}-n_j^{sub}||) n_j^{sub}),
\end{equation}
where $\Lambda(*)$ is the vector normalization function, and $W_s$ and $W_r$ are Gaussian weight functions, i.e., $W_{\sigma}(x) = exp(-x^2/(2\sigma^2))$, representing the spatial similarity and normal similarity recepectively between a pair of points. Standard deviations $\sigma_s$ and $\sigma_r$ used in $W_s$ and $W_r$ are parameters that need to be carefully tuned. Given two parameter sets $P_s = \{\sigma_{s_1}, \sigma_{s_2}, ...\}$ and $P_r = \{\sigma_{r_1}, \sigma_{r_2}, ...\}$, we can obtain several filtered normals using every combination of these two parameters. Together with the suboptimal one, we get a total of $X$ normals in the normal set of $p_i$, denoted as $N_f = \{ n_1, n_2, ... , n_X \} $.


\subsubsection{Height map patch construction:}
The point $p_i$ itself as well as one of its filtered normals $n_t$ defines a tangent plane, and the associated HMP is built on this plane. Suppose that we build a matrix with $m\times m$ bins that describes the local point position, and the center of the matrix is located at $p_i$. Similar as \cite{chen2019multi}, we fill each bin by weightedly averaging the height distances of points in a ball neighborhood of bin center $b_j$:
\begin{equation}
v_{b_j} = \frac{\sum_{p_k \in N_{ball}(b_j)} w(b_j, p_k) H(T(p_i, n_t), p_k)}{\sum_{p_k}w(b_j, p_k)},
\end{equation}
where $T(p_i, n_t)$ is the tangent plane defined by $p_i$ and $n_t$, $H(T(p_i, n_t), p_k)$ returns the signed distance from $p_k$ to the plane and $w(b_j, p_k) = exp(- \frac{||b_j-p_k||^2}{\sigma_d^2})$ is a spatial Gaussian weight function in which $\sigma_d$ is the residual bandwidth. Assembling all pairs of filtered normals and HMPs yields each point's MPD:
\begin{equation}
\textbf{MPD}_{i} = \{(n_1, \textbf{HMP}_1), (n_2, \textbf{HMP}_2), ..., (n_X, \textbf{HMP}_X)\}.
\end{equation}


\subsubsection{Consistency regardless of orientation:} To keep our MPD invariant to rotation, we need to take both normal invariance and HMP invariance into consideration. First, we apply a global rotation to the normals component of $\textbf{MPD}_{i}$ to make it invariant to rigid transformation. Specifically, we construct the rotation matrix $R_i$ by computing the normal tensor $T_i = \sum_{j=1}^X n_j \times n_j^T, n_j \in N_f$. The matrix $R_i$, defined by three eigenvectors (sorted by eigenvalues) of $T_i$, rotates all normals in $N_f$ to the Z-axis. Further, if one normal is in the direction of negative Z-axis, we reverse it to the positive one. The ground-truth normal is also applied by the same rotation matrix. For the HMPs component of $\textbf{MPD}_{i}$, their Z-axes of local coordinate systems are also rotated by the matrix $R_i$. The X-axis and Y-axis are computed by the cross product between the rotated normal and the two eigenvectors with smallest two eigenvalues.

%\subparagraph{MPD properties:}
%The MPD representation contains description both of normals and points position


\begin{table}[t]
	\centering
	%\setlength{\tabcolsep}{3.5mm}
	\begin{tabular}{c} %表格6列 全部居中显示
		\hline
		Transformation Network \\
		\hline 
		\hline
		Conv(3, 3, 64, P=1) + Relu \\
		Conv(3, 3, 128, P=1) + Relu  \\
		Maxpool(3, 3, S=1)  \\
		Conv(3, 3, 64, P=1) + Relu   \\
		Maxpool(3, 3, S=1)  \\
		Conv(3, 3, 64, P=1) + Relu  \\
		FC(256)  \\
		FC(128)  \\
		FC(k)  \\
		
		\hline
	\end{tabular}
	\hspace{5pt}
	\begin{tabular}{c}
		\hline
		gathering network \\
		\hline
		\hline
		
		$\{Y_j\}_{j=1}^{X}$ (input) \\
		FC(40) + Relu \\
		FC(3) \\
		\hline
	\end{tabular}
	\vspace{5pt}
	\caption{Architecture details of ablations.}
	\label{table:network}
\end{table}


\subsection{NH-Net architecture}
Our network architecture is outlined in Fig.~\ref{fig:pipeline} (the green part), which takes both normals and HMPs as input. First, we apply the cluster-based approach in \cite{wang2016mesh} to promote learning (see the detailed evaluation in the supplemental material). The key discussion is how to combine these two input feature from distinct data field (Section 4.2.2). Our network consists of two modules: a transformation module with three optional construction choices (Section 4.2.3) and a gathering module (Section 4.2.4). 
%The key idea is using HMP to learn a 3$\times$3 transformation matrix, which is used to consume the input normal and connect the two modules together. We then gather the separate branches of improving module, and output the final normal.

\subsubsection{Cluster-based method:}
Before training, we partition the training set into $K_c$ clusters via the k-means algorithm. It is performed on the normal components ($\{ N_f^i \}_{i=1}^n $) of MPD to cluster similar samples in one group. In each cluster, we train a separate NH-Net to map an MPD to its ground-truth counterpart. The network can then focus on a specific kind of geometric features and can intensively refine this kind of normals. In runtime test stage, a single MPD is distributed into one of these clusters if $||N_f^i - C_l|| \leq ||N_f^i - C_k||, \forall k$. Here, $C_k$ is the clustering center of the k-th cluster.

Furthermore, we evaluate the performance of different $K_c$ on our synthetic benchmark dataset, as shown in Fig.~\ref{fig:cluster}. We set $K_c = 4$ by default in all our experiment, unless stated otherwise. A larger $K_c$ improves the results slightly but heavily expands the network. 

\subsubsection{Framework overview}
In this section, we describe the general framework of our normal estimation network, which can be extended to a wide range of tasks with similar input features. Assume that, for a single estimation target, we have extracted two feature data from the raw input field, e.g., a feature matrix $M \in R^{m \times m}$ and a feature vector $V \in R^{n}$ including different information and even with distinct data type. In this ``double-input network'', in order to fully utilize the input feature fields, a connection module should be designed to combine these two data. Furthermore, the pair of $(M, V)$ can be extended to multi-scale version which contains more information for training. 

Separate networks, such as MLPs or convolutional layers, on distinct input data can result in incompatible high-dimensional feature concatenation, which may oppositely limit the learning ability.
The key idea behind our approach is that we use one feature matrix $M$ to learn an intermediate transformation target $T \in R^{n \times n}$ which should match the size of another input feature $V$, and apply the matrix product operator to obtain the higher-level feature $Y = T \cdot V$. Several architecture choices contructing the transformation $T$ will be discussed in Section 4.2.3 below. Then, we describe how to gather the combined features and output the final predicted result in Section 4.2.4.  

\subsubsection{Transformation network}
%Since the input $M$ and $V$ can be totally different features derived from different field, the common concatenation operation 
The intermediate transformation term $T$ should match the size of vector $V$, i.e., the column number of $T$ should equal to the row number of $V$, in order to apply the matrix product operation. The network module generating matrix $T$ is designed to extracting additional information and to refine the second input vector. In this work, we process each input $M$ using several convolutional layers and maxpool layers, followed by three fully connected layers (see Tab.\ref{table:network}). The output of this module can be a 1-dimensional vector of any size (length of $k$ in the output layer), which depends on the construction functions discussed below. Note that, in our normal estimation task, the input $M$ denotes a $m \times m$ height-map patch matrix and the input $V$ denotes a 3D normal vector.

\textbf{Rotation operator:}
In the field of 3D space, 3D rotation function is a commonly used operator which can be applied to normal vectors. To this end, we can learn a rotation matrix from the input martrix $M$ which parameterize the local point distribution related to $V$. Thus, vector $V$ can be rotated in the guidance of another feature. In particular, we use the transformation network to learn a quaternion, which means $k=4$ is set in the output dimension, and construct a $3 \times 3$ matrix $T$ from the unit quaternion.

\textbf{Transformation matrix:}
Another option that generates a transformation matrix does not require the quaternion for rotation. Intuitively, we set the output dimension as $k=9$ and simply reshape it to a $3 \times 3$ matrix, which is a more direct solution to combine the second feature vector similar to a rotation matrix. Note that, this construction function does not act the same as a rotation operator. An important distinction is that a transformation matrix is not designed strictly for rotating. This option can be viewed as a common 3D transformation applied to the input feature vector $V$.

\textbf{Weight matrix construction:}
In a more general situation, the intermediate transformaion $T$ can be any size as long as it matches the size of $V$, i.e., $T$ can be a $(x, n)$ weight matrix, rather that a regular $(n,n)$ one, which can also be combined with $V$ in the matrix product process. In this option, the transformation $T$ may capture more information than a simple $3 \times 3$ matrix, and have the ability (if $x > n$) to upgrade the input $V$ to a high-dimensional feature vector. We set $k = nx$ as the output dimension, and reshape it to a $(x, n)$ matrix $T$ which will be applied to $V$.

Also, if the two input feature are both 2-dimensional matrix with irregular size (row number $\neq$ column number), our framework still provides a solid connection as long as the column number of the first feature equal to the row number of the second one. This gives a general framework for this ``double-input network'' which leads to better result than the common concatenation solution.



%The HMP alone serves as the input at the start of the whole network. The improving module contains $X$ separate branches corresponding to the $X$ pairs in MPD, and each receives a single HMP and processes it using several convolutional layers and maxpool layers, outputting a $3 \times 3$ matrix $R_t^j$. Details of this module are shown in Fig.~\ref{fig:network} (the left part). The output matrix is regarded as a transformation matrix and will be used in the gathering module. This design of identical branches is chosen to better preserve local features associated with the varying parameters of previous bilateral filters.
%Note that each HMP owns a separate learning branch. Thus, totally $X$ HMP-based improving modules are included which are designed to preserve local features associated with the varying parameters of previous bilateral filters.
%Each branch is independently designed to preserve local features associated with varying parameters of previous bilateral filters and prevent averaging effects later in our gathering module.


\subsubsection{Gathering module}
In our normal estimation network, the input feature $M$ denotes the $m \times m$ HMP and feature $V$ denotes the normal vector in MPD. And with the multi-scale scheme, we have $X$ pairs of $M$ and $V$ designed for the network input.
For each pair of input, we process it using a separate module and obtain the transformed features $\{Y_j\}_{j=1}^X$, which combines the two kind of input features. Then, we concatenate these vectors and feed them to the gathering module (see Tab.\ref{table:network}), which outputs the final predicted normal $N^* = (N_x, N_y, N_z)$. Batch normalization and ReLU are included in each layer of this module.
%After obtaining outputs $\{R_t^j\}_{j=1}^X$ from the improving modules, our network applies each $3 \times 3$ matrix to its corresponding normal and gets a new vector $c_j = R_t^j n_j$. The standardization version of these vectors, processed by one layer of batch normalization, is fed to the gathering module. This module is a single-layer fully connected network which outputs the ultimate normal $N^* = (N_x, N_y, N_z)$.

%\subparagraph{Clustering via k-means:}
%For MPDs in the training dataset, we first separate them into $K_c$ clusters via a k-means algorithm on the domain of $N_f$ in MPD. Then a NH-Net is trained for each cluster. The clustering method can detect similar geometric features among all training samples, especially  it segregates fine normals from the bad ones. In runtime test stage, a single MPD is divided into one of these clusters if $||N_f^i - C_l|| < ||N_f^i - C_k||, \forall k$. Here, $C_k$ is the clustering center of the k-th cluster.


\subsubsection{Loss function}
We train the network by minimizing the MSE loss between the output normal $N^*$ and its ground truth $\hat{N}$:
\begin{equation}
Loss = || \Lambda(N^*) - \hat{N} ||^2 + \lambda E_{reg},
\end{equation}
Here, $\Lambda(*)$ is the vector normalization function, $E_{reg}$ is the commonly-used $L_2$ regularization term to avoid overfitting and $\lambda = 0.02$ is used.

\iffalse
\begin{figure*}
	\begin{center}
		\includegraphics[clip, trim=1cm 7cm 1cm 7cm, width=1\textwidth]{fig/benchmark/normal_cmp1.pdf}
	\end{center}
	\caption{The average angular errors (degree) of compared methods on the synthetic benchmark dataset.}
	\label{fig:benchmark:normal_cmp}
\end{figure*}
\fi

\begin{figure*}
	\begin{center}
		\includegraphics[width=0.99\linewidth]{fig/benchmark/normal_cmp.pdf} 	
	\end{center}
	\vspace{-8pt}
	\caption{The average angular errors (degree) of compared methods on the synthetic benchmark dataset.}
	\label{fig:benchmark:normal_cmp}
\end{figure*}


\begin{figure*}
	\centering
	\includegraphics[width=0.12\linewidth]{fig/boy/input.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/pca.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/HF.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/HoughCNN.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/pcpnet.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/PCV.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/nesti.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/Ours.eps}
	% \vspace{-10pt}
	\subfigure[Input]{
		\label{fig:cone:input} %% label for first subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/input.eps}}\hspace{-5pt}
	\subfigure[PCA \cite{hoppe1992surface}]{
		\label{fig:cone:pca} %% label for second subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/pca.eps}}\hspace{-5pt}
	\subfigure[HF \cite{boulch2012fast}]{
		\label{fig:cone:HF} %% label for second subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/HF.eps}}\hspace{-5pt}
	\subfigure[HoughCNN \cite{boulch2016deep}]{
		\label{fig:cone:HoughCNN} %% label for second subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/HoughCNN.eps}}\hspace{-5pt}
	\subfigure[PCPNet \cite{GuerreroEtAl:PCPNet:EG:2018}]{
		\label{fig:cone:pcpnet} %% lael for second subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/pcpnet.eps}}\hspace{-5pt}
	\subfigure[PCV \cite{zhang2018multi}]{
		\label{fig:cone:PCV} %% label for first subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/PCV.eps}}\hspace{-5pt}
	\subfigure[Nesti-Net \cite{Ben-ShabatLF19}]{
		\label{fig:cone:nesti} %% label for first subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/nesti.eps}}\hspace{-5pt}
	\subfigure[Ours]{
		\label{fig:cone:ours} %% label for first subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/Ours.eps}}
	
	\caption{Visual comparison of estimated normals by different methods on two real scanned models from \cite{wang2016mesh}.}%The average normal errors are: $11.5^{\circ}$, $14.2^{\circ}$, $14.6^{\circ}$, $11.6^{\circ}$, $11.1^{\circ}$, and $\textbf{8.8}^{\circ}$, respectively.%
	\label{fig:real_boy}
\end{figure*}


\section{Evaluation}
In this section, we evaluate the models using different transformation modules for several benchmark dataset: synthetic models, real-scan models and indoor scene point clouds. Detailed network architecture and visual normal results are provided. In addition, we show that our NH-Net is able to improve other deep-learning normal estimation network, and refine their results.

\subsection{Experiments on synthetic data}
\subsubsection{Dataset}
We use the training set from \cite{wang2016mesh} to train the network. The dataset contains 21 synthetic triangular mesh models with varying sampling density and is manually divided into three categories: CAD-like models, smooth models and feature-rich models. Each type is collected from shapes representing different challenging geometric features. We simply extract the mesh vertices as point samples and the mesh normals as ground-truth normals in order to preserve the original features for training. We follow the experimental settings of \cite{zhang2018multi}. To generate noisy inputs, we introduce Gaussian noise for each point cloud with a standard deviation of $0.1\%$, $0.2\%$ and $0.3\%$ of the diagonal length of the bounding box. The final training dataset contains 1.5M points from 63 noisy point clouds, in which $20\%$ of point samples are used for validation.

For test set, we collect additional point clouds apart from the test set of \cite{wang2016mesh} from \cite{zhang2018multi}. Similarly, the test set includes 4 categories: SharpFeature, SmoothSurface, RichFeature and BigNoise category, in which there are 11, 8, 8 and 8 models respectively. For data augmentation, each point cloud in the SharpFeature and SmoothSurface categories is perturbed by Gaussian noise with a standard deviation of $0.05\%$, $0.1\%$ and $0.15\%$ of the diagonal length of the bounding box. For the RichFeaure category, $0.05\%$, $0.1\%$, $0.15\%$ and $0.2\%$ noise are introduced and $0.2\%$, $0.3\%$, $0.4\%$ and $0.5\%$ for the BigNoise category. Our test set contains totally 121 point clouds with over 3M point samples.

%\[ \textbf{NG}_{p_i} = \{n_f | p_i \text{ is a vertex of face } f\}\]

\subsubsection{Architecture}
First, suboptimal normal is computed for each point (Section 3) as a preparation for the network training. We also provide these normal results in Fig. for a fair comparison. The neighborhood size set K is the most practical parameter in MFPS process. We set $K = 50, 100, 150$ empirically. For BigNoise category in test stage, we double the size to $K = 100, 200, 300$.

When constructing MPDs, the parameter pairs used in bilateral filtering are set as $P_s = \{\overline{l}_d, 2\overline{l}_d\}$ and $P_r = \{0.1, 0.2, 0.35, 0.5\}$, where $\overline{l}_d$ is the average distance between points. Thus, together with the suboptimal normal, MPD includes 9 pairs of normal and HMP, i.e., there are 9 separate branches of transformation module to connect these two input data. For the HMP construction, we use a $7\times7$ ($m = 7$) height-map grid.

The network architecture for NH-Net normal estimation is showed in Tab.~\ref{table:network}, in which the transformation module is repeated for each pair of the two inputs. We process the HMP (input matrix $M$ of size $7 \times 7$) using convolutional layers followed by fully-connected layers (256, 128, k), which naturally matches its grid-like data struction. Batch normalization and ReLU are included in the fully-connected layers. Dropout with a keep probability of $0.3$ is introduced in the last two fully-connected layers. To fit other type of matrix $M$ into our framework, MLPs or other deep network architectures can also be used. The output dimension $k$ depends on the construction choices used, and we test all three construction functions mentioned in the previous sections. In the third option, $k = 8 \times 3$ is set empirically.

The gathering module we used is a two-layer fully-connected network, which collects outputs from separate transformation networks. We find in the experiment that this simple design is able to gather information which is already combined by the previous modules. Similar to the transformation networks, batch normalization and dropout layers are included in each layer.

\subsubsection{Training}
We use SGD optimizer with learning rate $0.0001$, and we do not use learning rate decay in all epochs. The batch size is 512 for all training clusters and the momentum for batch normalization is $0.9$. We use PyTorch implementation and train the networks on a RTX 2080 Ti GPU.

\begin{table*}
	\centering
	\small
	%\footnotesize
	\setlength{\tabcolsep}{3.5mm}
	%\setlength{\arrayrulewidth}{0.7pt}
	\begin{tabular}{c c c c c c} %表格6列 全部居中显示
		\hline
		Category & BigNoise & SharpFeature & RichFeature & SmoothSurface & Average \\
		\hline 
		PCA \cite{hoppe1992surface} & $8.53^{\circ}$  & $8.70^{\circ}$  & $6.94^{\circ}$ & $8.04^{\circ}$ & $8.05^{\circ}$ \\
		HF \cite{boulch2012fast} & $11.73^{\circ}$  & $5.26^{\circ}$  & $5.81^{\circ}$ & $3.87^{\circ}$ & $6.67^{\circ}$ \\
		HoughCNN1s & $8.76^{\circ}$  & $5.40^{\circ}$  & $6.00^{\circ}$ & $5.05^{\circ}$ & $6.30^{\circ}$ \\
		HoughCNN3s & $8.61^{\circ}$  & $5.52^{\circ}$  & $5.61^{\circ}$ & $5.89^{\circ}$ & $6.41^{\circ}$ \\
		HoughCNN5s & $10.78^{\circ}$  & $6.48^{\circ}$  & $6.46^{\circ}$ & $7.40^{\circ}$ & $7.78^{\circ}$ \\
		PCPNet-ss & $9.61^{\circ}$  & $12.84^{\circ}$  & $6.84^{\circ}$ & $12.84^{\circ}$ & $10.53^{\circ}$ \\
		PCPNet-ms & $9.09^{\circ}$  & $7.90^{\circ}$  & $5.97^{\circ}$ & $5.27^{\circ}$ & $7.06^{\circ}$ \\
		LRR \cite{zhang2013point} & $5.77^{\circ}$  & $4.39^{\circ}$  & $4.86^{\circ}$ & $4.66^{\circ}$ & $4.92^{\circ}$ \\
		PCV \cite{zhang2018multi} & $5.89^{\circ}$  & $4.59^{\circ}$  & $4.80^{\circ}$ & $3.97^{\circ}$ & $4.81^{\circ}$ \\
		Nesti-Net \cite{Ben-ShabatLF19} & $5.65^{\circ}$  & $4.28^{\circ}$  & $4.62^{\circ}$ & $4.20^{\circ}$ & $4.69^{\circ}$ \\
		MFPS & $5.97^{\circ}$  & $4.36^{\circ}$  & $4.82^{\circ}$ & $4.10^{\circ}$ & $4.81^{\circ}$ \\
		Ours-Rot & $5.50^{\circ}$  & $3.79^{\circ}$  & $4.45^{\circ}$ & $3.67^{\circ}$ & $4.35^{\circ}$ \\
		Ours-Trans & $5.49^{\circ}$  & $3.75^{\circ}$  & $4.42^{\circ}$ & $3.64^{\circ}$ & $4.32^{\circ}$ \\
		Ours-Weight & $5.47^{\circ}$  & $3.73^{\circ}$  & $4.39^{\circ}$ & $3.63^{\circ}$ & $4.30^{\circ}$ \\
		\hline
	\end{tabular}
	\caption{Comparison of normal estimation errors on synthetic benchmark dataset.}
	\label{table:sys_cmp}
\end{table*}

\subsubsection{Results}
To quantitatively testify our method, we use the mean angular errors (degrees) between estimated normals and their ground-truth counterparts as an evaluation metric, which is typically used for normal accuracy comparison. Fig.~\ref{label} shows the results on the synthetic dataset. We compare our method, including MFPS alone and the full pipeline (MFPS+NH-Net) using three alternative, with several traditional and deep-learning state-of-the-arts: PCA \cite{hoppe1992surface}, HF \cite{boulch2012fast}, LRR \cite{zhang2013point}, PCV \cite{zhang2018multi}, HoughCNN \cite{boulch2016deep}, PCPNet \cite{GuerreroEtAl:PCPNet:EG:2018} and Nesti-Net \cite{Ben-ShabatLF19}. We retrained HoughCNN, PCPNet and Nesti-Net on our own dataset. In addition, HoughCNN has three versions with different scales and PCPNet has single-scale and multi-scale versions. We evaluate all these versions. For the above methods, we set a same neighborhood size $K=100$ for three categories: SharpFeature, RichFeature and SmoothSurface.
In particular, the HoughCNN3s considers 3 scales, $K = 50,100,200$, which is recommended in their paper. For the BigNoise category, we double the neighborhood size, i.e., $K = 100,200,400$ for HoughCNN3s, and $K=200$ for other single scale methods. Besides, HoughCNN5s considers 5 scales, $K = 32,64,128,256,512$, for all categories. All other parameters are set by default values.
%The filtering neighborhood size is $K = 70$.

%For clustering, we find in our experiment that 2 clusters are enough for a good result. By default, the cluster number is set as $K_c = 4$, balancing the computational cost and performance well.


\subsection{Experiments on real scans}
Our method is also tested on real point cloud dataset scanned by Microsoft Kinect v1 from \cite{wang2016mesh}. We show visual comparisons of estimated normals rendered in RGB color images in Fig.~\ref{fig:real_boy}. The real scan data reveals more challenges, such as the fluctuation on flat surface, originated from the projection process of Kinect camera. The non-Gaussian and discontinuous noise interferes the estimator against recovering the underlying surface. By training on such scanned data (from \cite{wang2016mesh}), our NH-Net is able to distinguish geometric features from undesired scanning noise. Meanwhile, as shown in Tab.~\ref{table:errors}, our method performs better than all other methods in terms of the normal accuracy.
%However, the ground-truth normals in real point clouds are not easy-available. Instead, with the help of the sampling strategy from \cite{wang2016mesh} by first obtaining the high-resolution scanned result $M^h$, and then projecting the noisy scaned vertex onto its nearest point on the high-resolution $M^h$ via rigid ICP. We finally get the ground-truth mesh $M^g$ that has the same mesh connectivity with the noisy one $M^n$. $\{M^n, M^g\}$ serves as the noisy input and its ground-truth counterpart.

Furthermore, we show qualitative results of several real scans of indoor scenes provided by NYU Depth V2 \cite{silberman2012indoor}. From Fig.~\ref{fig:indoor}, PCA, HF, HoughCNN and PCV, can preserve tiny details but with the price of retaining noise (see from Fig.~\ref{fig:indoor:pca} to \ref{fig:indoor:PCV}). Nesti-Net can well smooth the noisy surface, but over-smooths geometric features (Fig.~\ref{fig:indoor:nesti}). Please note we train all networks by the same dataset for a fair comparison. 

We also report the time performance of our method and the compared methods in Tab. \ref{table:errors}. The running time of our approach is the total testing time including all steps. 

\begin{table}[t]
	\centering
	\small
	%\setlength{\tabcolsep}{3.5mm}
	\begin{tabular}{c|c}

		concat & residual\\ 
		\hline 
		$\textbf{HMP}_j$ & $\textbf{HMP}_j$ \\
		Conv(3, 3, 64, P=1) + Relu & Conv(3, 3, 64, P=1) + Relu \\
		Conv(3, 3, 128, P=1) + Relu & Conv(3, 3, 64, P=1) + Relu \\
		Maxpool(3, 3, S=1) & Maxpool(3, 3, S=1) \\
		Conv(3, 3, 64, P=1) + Relu & Conv(3, 3, 64, P=1) + Relu \\
		Maxpool(3, 3, S=1) & Maxpool(3, 3, S=1) \\
		Conv(3, 3, 64, P=1) + Relu & Conv(3, 3, 64, P=1) + Relu \\
		FC(256) & FC(256) \\
		FC(128) & FC(128) \\
		FC(64) & FC(3) \\
		\hline
		$Y_j = (T, n_j(3, 64, 64))$ & $Y_j = T + n_j$ \\
		\hline
		$\{Y_j\}_{j=1}^{X}$ & $\{Y_j\}_{j=1}^{X}$ \\
		FC(512) & FC(64) \\
		FC(256) & FC(32) \\
		FC(3) & FC(3) \\
		
	\end{tabular}
	\caption{Ablation architecture details for the variant concat and residual. First, each HMP is processed separately to obtain a intermediate feature $T$, similar to the proposed NH-Net. Then, feature vector $V$($n_j$) is combined differently for $Y_j$, which is then fed into the output module.}
	\label{table:ablation}
\end{table}

\subsection{Experiments on different learning schemes}
In this section, we explain some of the architecture choices used in the network. Compared with the works in \cite{wang2016mesh}, we introduce additional HMP matrix as a second input feature apart from the filtered normals. The suboptimal normal for each point, processed by multi-scale bilateral filtering, collect information from its local neighborhood and can well handle the main challenges of high-level noise and sharp features. However, training that solely relies on normal vectors may ignore the basic point distribution, which can be extracted by computing the HMPs. We test our network by using only normal feature and only HMP feature as input, and outputting the predicted normal. The normal-net takes normal component of MPD as input, and processes it using gathering module architecture (64, 32, 3). Similarly, the HMP-net uses all HMPs of the filtered normals, and is composed of convolutional layers (64, 64, 128) followed by fully-connected layers (512, 256, 128, 3). Fig.~\ref{label} shows the results of the two ablations on synthetic dataset, which denotes that input of single data type leads to a lower estimation accuracy.

The key idea behind our approach is the designed transformation module which tries to learn a transformation $T$ in order to combine the two feature matrices. We find the common concatenation operator applied on multi-scale inputs or even distinct input data can not fully promote the network ability and process the input features. The practice that combines two features using matrix product with transformation $T$ shows its advantages compared with other learning schemes \ref{label}. To this end, we design two ablations of our network: 

$\bullet$ concat - Just simply concatenate two features obtained separately from normal and HMP component and process it using fully-connected layers (512, 256, 128, 3). The normal feature is obtained by additional fully-connected layers (3, 64, 64); see Table \ref{table:ablation} left.

$\bullet$ residual - Replace the matrix $T$ by a single vector with the same size of $V$, which learns the residual (noise in point cloud) between input and ground-truth. The intermediate feature $Y$ is obtained by $V$ plus the residual; see Table \ref{table:ablation} right.

Inspired by \cite{wang2016mesh}, NH-Net uses a cluster-based network architecture to promote learning. The cluster-based scheme devide the input samples into $K_c$ clusters before training, which is vital to the final predicted results (see Fig.~\ref{label}). Note that, in all our experiments including the variants of the proposed network, we set $K_c = 4$ by default. A larger $K_c$ slightly improves the performance but heavily expands the network. Furthermore, we show the comparison between input normals (suboptimal normal by MFPS) and the final normals within each cluster in Fig.~\ref{label}. This pre-processing scheme divide all points into separate clusters with similar feature, lowering the learning difficulty with multiple specific networks. Also, we see the network achieve better improvements on two of the clusters, which denotes the better performance in regions with high-level noise, where the initial normals are not accurate. 


\subsection{Application}
As known, well-estimated normals can boost the effect of many point cloud processing tasks, like denoising and surface reconstruction. To further verify the advantages of our method, we show denoising results using the same point updating algorithm, yet based on the normal results estimated by different methods.

Denote that $\mathcal N_i$ is the ball neighborhood of $p_i$, we here provide an algorithm to update point positions under the guidance of estimated normals, which is able to remove noise and recover sharp features:
\begin{equation}
p_i' = p_i + \gamma_i \sum_{{p}_{j} \in \mathcal N_i} (p_j-p_i)(w_\sigma(n_i,n_j) n_i^T n_i + \lambda n_j^T n_j).
\end{equation}
where $w_\sigma(n_i,n_j) = exp(-\frac{||n_i-n_j||^2}{\sigma ^2})$ is a weight function, $\lambda = 0.5$ is a tradeoff parameter and $\gamma_i$ is step size set to $\frac{1}{3|\mathcal N_i|}$ by default. To prevent points from accumulating around edges, we keep the neighboring information unchanged in all iterations \cite{lu2018low}. The iteration number is set to 20 in our experiment.

We demonstrate visual quality of the denoising results and their reconstruction results (see from Fig. \ref{fig:block}). Our normal results help produce the most faithful denoising and reconstruction results.
%in terms of sharp feature recovery (see from block model in the first and second rows) and detail recovery (see from armadillo model in the third and bottom rows). 


==> network.tex <==
\section{NH-Net}
In this section, we introduce the learning part in our algorithm pipeline. The network architecture is outlined in Fig. \ref{fig:pipeline} (the purple and green parts). First, we introduce a multi-scale descriptor, called MPD, and then explain how to feed it into the next two-stage learning module which spits out the final normal. The details are followed.

\subsection{MPD: multi-scale point descriptor}
As known, the input data of a neural network should be in a structural format. Inspired by the work in Wang et al. \cite{wang2016mesh}, for each point, we define its MPD by $X$ pairs of filtered normal plus local HMP to collaboratively enhance the learning effect. Filtered normals at each point are computed by bilateral filtering based on the normals estimated in Sec. 4, and the HMPs are constructed according to the corresponding filtered normals.

\vspace{-7pt}
\paragraph{Multi-scale bilateral filters:}
We give a brief introduction to the commonly-used bilateral filters \cite{jones2004normal}. Denote the neighborhood of $p_i$ as $N_i$, and the normal at each point as $n_i^{sub}$. The filtered normal can be defined as:
\begin{equation}
n_i = \Lambda(\sum_{{p}_{j}\in N_i} W_s(||p_i-p_j||) W_r(||n_i^{sub}-n_j^{sub}||) n_j^{sub}),
\end{equation}
where $\Lambda(*)$ is the vector normalization function, and $W_s$ and $W_r$ are Gaussian weight functions, \ie, $W_{\sigma}(x) = exp(-x^2/(2\sigma^2))$, representing the spatial similarity and normal similarity respectively between a pair of points. Standard deviations $\sigma_s$ and $\sigma_r$ used in $W_s$ and $W_r$ are parameters that need to be carefully tuned. Given two parameter sets $P_s = \{\sigma_{s_1}, \sigma_{s_2}, ...\}$ and $P_r = \{\sigma_{r_1}, \sigma_{r_2}, ...\}$, we can obtain several filtered normals using every combination of these two parameters. Together with the suboptimal one, we get a total of $X$ normals in the normal set of $p_i$, denoted as $N_f = \{ n_1, n_2, ... , n_X \} $.

\vspace{-7pt}
\paragraph{Height map patch construction:}
The point $p_i$ itself as well as one of its filtered normals $n_t$ defines a tangent plane, and the associated HMP is built on this plane. Suppose that we build a matrix with $m\times m$ bins that describes the local point position, and the center of the matrix is located at $p_i$. Similar as \cite{chen2019multi}, we fill each bin by weighted averaging the height distances of points in a ball neighborhood of bin center $b_j$:
\begin{equation}
v_{b_j} = \frac{\sum_{p_k \in N_{ball}(b_j)} w(b_j, p_k) H(T(p_i, n_t), p_k)}{\sum_{p_k}w(b_j, p_k)},
\end{equation}
where $T(p_i, n_t)$ is the tangent plane defined by $p_i$ and $n_t$, $H(T(p_i, n_t), p_k)$ returns the signed distance from $p_k$ to the plane and $w(b_j, p_k) = exp(- \frac{||b_j-p_k||^2}{\sigma_d^2})$ is a spatial Gaussian weight function in which $\sigma_d$ is the residual bandwidth. Assembling all pairs of filtered normals and HMPs yields each point's MPD:
\begin{equation}
\textbf{MPD}_{i} = \{(n_1, \textbf{HMP}_1), (n_2, \textbf{HMP}_2), ..., (n_X, \textbf{HMP}_X)\}.
\end{equation}

\vspace{-7pt}
\paragraph{Consistency regardless of orientation:} To keep our MPD invariant to rotation, we need to take both normal invariance and HMP invariance into consideration. First, we apply a global rotation to the normals component of $\textbf{MPD}_{i}$ to make it invariant to rigid transformation. Specifically, we construct the rotation matrix $R_i$ by computing the normal tensor $T_i = \sum_{j=1}^X n_j \times n_j^T, n_j \in N_f$. The matrix $R_i$, defined by three eigenvectors (sorted by eigenvalues) of $T_i$, rotates all normals in $N_f$ to the Z-axis. Further, if one normal is in the direction of negative Z-axis, we reverse it to the positive one. The ground-truth normal is also applied by the same rotation matrix. For the HMPs component of $\textbf{MPD}_{i}$, their Z-axes of local coordinate systems are also rotated by the matrix $R_i$. The X-axis and Y-axis are computed by the cross product between the rotated normal and the two eigenvectors with smallest two eigenvalues.

%\subparagraph{MPD properties:}
%The MPD representation contains description both of normals and points position


\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.9\linewidth]{network.pdf}
	\end{center}
	\caption{The branch of HMP-based improving module (left), and the gathering module (right).}
	\label{fig:network}
\end{figure}

\subsection{NH-Net architecture}
Our network architecture is outlined in Fig.~\ref{fig:pipeline} (the green part), which takes both normals and HMPs as input. First, we apply the cluster-based approach in \cite{wang2016mesh} to promote learning (see the detailed evaluation in the supplemental material). Our network consists of two modules: an HMP-based improving module and a gathering module. The key idea is using HMP to learn a 3$\times$3 transformation matrix, which is used to consume the input normal and connect the two modules together. We then gather the separate branches of improving module, and output the final normal.

\vspace{-7pt}
\paragraph{HMP-based improving module:}
The HMP alone serves as the input at the start of the whole network. The improving module contains $X$ separate branches corresponding to the $X$ pairs in MPD, and each receives a single HMP and processes it using several convolutional layers and maxpool layers, outputting a $3 \times 3$ matrix $R_t^j$. Details of this module are shown in Fig.~\ref{fig:network} (the left part). The output matrix is regarded as a transformation matrix and will be used in the gathering module. This design of identical branches is chosen to better preserve local features associated with the varying parameters of previous bilateral filters.
%Note that each HMP owns a separate learning branch. Thus, totally $X$ HMP-based improving modules are included which are designed to preserve local features associated with the varying parameters of previous bilateral filters.
%Each branch is independently designed to preserve local features associated with varying parameters of previous bilateral filters and prevent averaging effects later in our gathering module.

\vspace{-7pt}
\paragraph{Gathering module:}
After obtaining outputs $\{R_t^j\}_{j=1}^X$ from the improving modules, our network applies each $3 \times 3$ matrix to its corresponding normal and gets a new vector $c_j = R_t^j n_j$. The standardization version of these vectors is fed to the gathering module. This module is a single-layer fully connected network which outputs the ultimate normal $N^* = (N_x, N_y, N_z)$.

%\subparagraph{Clustering via k-means:}
%For MPDs in the training dataset, we first separate them into $K_c$ clusters via a k-means algorithm on the domain of $N_f$ in MPD. Then a NH-Net is trained for each cluster. The clustering method can detect similar geometric features among all training samples, especially  it segregates fine normals from the bad ones. In runtime test stage, a single MPD is divided into one of these clusters if $||N_f^i - C_l|| < ||N_f^i - C_k||, \forall k$. Here, $C_k$ is the clustering center of the k-th cluster.

\vspace{-7pt}
\paragraph{Loss function:}
We train the network by minimizing the MSE loss between the output normal $N^*$ and its ground truth $\hat{N}$:
\begin{equation}
Loss = || \Lambda(N^*) - \hat{N} ||^2 + \lambda E_{reg},
\end{equation}
Here, $\Lambda(*)$ is the vector normalization function, $E_{reg}$ is the commonly-used $L_2$ regularization term to avoid overfitting and $\lambda = 0.02$ is used.

\iffalse
\begin{figure*}
	\begin{center}
		\includegraphics[clip, trim=1cm 7cm 1cm 7cm, width=1\textwidth]{fig/benchmark/normal_cmp1.pdf}
	\end{center}
	\caption{The average angular errors (degree) of compared methods on the synthetic benchmark dataset.}
	\label{fig:benchmark:normal_cmp}
\end{figure*}
\fi

\begin{figure*}
	\begin{center}
		\includegraphics[width=0.99\linewidth]{fig/benchmark/normal_cmp.pdf} 	
	\end{center}
	\vspace{-8pt}
	\caption{The average angular errors (degree) of compared methods on the synthetic benchmark dataset.}
	\label{fig:benchmark:normal_cmp}
\end{figure*}


\begin{figure*}
	\centering
	\includegraphics[width=0.12\linewidth]{fig/boy/input.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/pca.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/HF.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/HoughCNN.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/pcpnet.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/PCV.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/nesti.eps}%\hspace{-5pt}
	\includegraphics[width=0.12\linewidth]{fig/boy/Ours.eps}
	% \vspace{-10pt}
	\subfigure[Input]{
		\label{fig:cone:input} %% label for first subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/input.eps}}\hspace{-5pt}
	\subfigure[PCA \cite{hoppe1992surface}]{
		\label{fig:cone:pca} %% label for second subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/pca.eps}}\hspace{-5pt}
	\subfigure[HF \cite{boulch2012fast}]{
		\label{fig:cone:HF} %% label for second subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/HF.eps}}\hspace{-5pt}
	\subfigure[HoughCNN \cite{boulch2016deep}]{
		\label{fig:cone:HoughCNN} %% label for second subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/HoughCNN.eps}}\hspace{-5pt}
	\subfigure[PCPNet \cite{GuerreroEtAl:PCPNet:EG:2018}]{
		\label{fig:cone:pcpnet} %% lael for second subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/pcpnet.eps}}\hspace{-5pt}
	\subfigure[PCV \cite{zhang2018multi}]{
		\label{fig:cone:PCV} %% label for first subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/PCV.eps}}\hspace{-5pt}
	\subfigure[Nesti-Net \cite{Ben-ShabatLF19}]{
		\label{fig:cone:nesti} %% label for first subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/nesti.eps}}\hspace{-5pt}
	\subfigure[Ours]{
		\label{fig:cone:ours} %% label for first subfigure
		\includegraphics[width=0.12\linewidth]{fig/girl/Ours.eps}}
	
	\caption{Visual comparison of estimated normals by different methods on two real scanned models from \cite{wang2016mesh}.}%The average normal errors are: $11.5^{\circ}$, $14.2^{\circ}$, $14.6^{\circ}$, $11.6^{\circ}$, $11.1^{\circ}$, and $\textbf{8.8}^{\circ}$, respectively.%
	\label{fig:real_boy}
\end{figure*}

\subsection{Training details}
\paragraph{Training dataset:}
We use the dataset from \cite{wang2016mesh} for training. The training set is built from synthetic triangular mesh models, including point samples and normals.
%We extract the mesh vertices as point samples and use normals of mesh faces as the ground truth normal for each point.

%\[ \textbf{NG}_{p_i} = \{n_f | p_i \text{ is a vertex of face } f\}\]

The ground-truth point clouds consist of 21 models including 6 CAD models, 8 smooth models and 7 feature-rich models. To generate the noisy inputs, we introduce Gaussian noise for each point cloud with a standard deviation of $0.1\%$, $0.2\%$ and $0.3\%$ of the diagonal length of the bounding box. The final training dataset contains 1.5M points from 63 noisy point clouds.

\vspace{-7pt}
\paragraph{Parameters:}
When constructing MPDs, the parameter pairs used in bilateral filtering are set as $P_s = \{\overline{l}_d, 2\overline{l}_d\}$ and $P_r = \{0.1, 0.2, 0.35, 0.5\}$, where $\overline{l}_d$ is the average distance between points. Thus, together with the suboptimal normal, MPD includes 9 pairs of normal and HMP, \ie, there are 9 separate branches in the HMP-based improving module. For the HMP construction, we use a $7\times7$ ($m = 7$) height-map grid. We train the network using PyTorch on a single NVIDIA Geforce RTX 2080 Ti GPU.
%The filtering neighborhood size is $K = 70$.

%For clustering, we find in our experiment that 2 clusters are enough for a good result. By default, the cluster number is set as $K_c = 4$, balancing the computational cost and performance well.

